Demystifying Deception Technology:A Survey

Deception boosts security for systems and components by denial, deceit, misinformation, camouflage and obfuscation. In this work an extensive overview of the deception technology environment is presented. Taxonomies, theoretical backgrounds, psychological aspects as well as concepts, implementations, legal aspects and ethics are discussed and compared.

==> gradlew <==
#!/usr/bin/env bash

##############################################################################
##
##  Gradle start up script for UN*X
##
##############################################################################

# Attempt to set APP_HOME
# Resolve links: $0 may be a link
PRG="$0"
# Need this for relative symlinks.
while [ -h "$PRG" ] ; do
    ls=`ls -ld "$PRG"`
    link=`expr "$ls" : '.*-> \(.*\)$'`
    if expr "$link" : '/.*' > /dev/null; then
        PRG="$link"
    else
        PRG=`dirname "$PRG"`"/$link"
    fi
done
SAVED="`pwd`"
cd "`dirname \"$PRG\"`/" >/dev/null
APP_HOME="`pwd -P`"
cd "$SAVED" >/dev/null

APP_NAME="Gradle"
APP_BASE_NAME=`basename "$0"`

# Add default JVM options here. You can also use JAVA_OPTS and GRADLE_OPTS to pass JVM options to this script.
DEFAULT_JVM_OPTS=""

# Use the maximum available, or set MAX_FD != -1 to use that value.
MAX_FD="maximum"

warn ( ) {
    echo "$*"
}

die ( ) {
    echo
    echo "$*"
    echo
    exit 1
}

# OS specific support (must be 'true' or 'false').
cygwin=false
msys=false
darwin=false
nonstop=false
case "`uname`" in
  CYGWIN* )
    cygwin=true
    ;;
  Darwin* )
    darwin=true
    ;;
  MINGW* )
    msys=true
    ;;
  NONSTOP* )
    nonstop=true
    ;;
esac

CLASSPATH=$APP_HOME/gradle/wrapper/gradle-wrapper.jar

# Determine the Java command to use to start the JVM.
if [ -n "$JAVA_HOME" ] ; then
    if [ -x "$JAVA_HOME/jre/sh/java" ] ; then
        # IBM's JDK on AIX uses strange locations for the executables
        JAVACMD="$JAVA_HOME/jre/sh/java"
    else
        JAVACMD="$JAVA_HOME/bin/java"
    fi
    if [ ! -x "$JAVACMD" ] ; then
        die "ERROR: JAVA_HOME is set to an invalid directory: $JAVA_HOME

Please set the JAVA_HOME variable in your environment to match the
location of your Java installation."
    fi
else
    JAVACMD="java"
    which java >/dev/null 2>&1 || die "ERROR: JAVA_HOME is not set and no 'java' command could be found in your PATH.

Please set the JAVA_HOME variable in your environment to match the
location of your Java installation."
fi

# Increase the maximum file descriptors if we can.
if [ "$cygwin" = "false" -a "$darwin" = "false" -a "$nonstop" = "false" ] ; then
    MAX_FD_LIMIT=`ulimit -H -n`
    if [ $? -eq 0 ] ; then
        if [ "$MAX_FD" = "maximum" -o "$MAX_FD" = "max" ] ; then
            MAX_FD="$MAX_FD_LIMIT"
        fi
        ulimit -n $MAX_FD
        if [ $? -ne 0 ] ; then
            warn "Could not set maximum file descriptor limit: $MAX_FD"
        fi
    else
        warn "Could not query maximum file descriptor limit: $MAX_FD_LIMIT"
    fi
fi

# For Darwin, add options to specify how the application appears in the dock
if $darwin; then
    GRADLE_OPTS="$GRADLE_OPTS \"-Xdock:name=$APP_NAME\" \"-Xdock:icon=$APP_HOME/media/gradle.icns\""
fi

# For Cygwin, switch paths to Windows format before running java
if $cygwin ; then
    APP_HOME=`cygpath --path --mixed "$APP_HOME"`
    CLASSPATH=`cygpath --path --mixed "$CLASSPATH"`
    JAVACMD=`cygpath --unix "$JAVACMD"`

    # We build the pattern for arguments to be converted via cygpath
    ROOTDIRSRAW=`find -L / -maxdepth 1 -mindepth 1 -type d 2>/dev/null`
    SEP=""
    for dir in $ROOTDIRSRAW ; do
        ROOTDIRS="$ROOTDIRS$SEP$dir"
        SEP="|"
    done
    OURCYGPATTERN="(^($ROOTDIRS))"
    # Add a user-defined pattern to the cygpath arguments
    if [ "$GRADLE_CYGPATTERN" != "" ] ; then
        OURCYGPATTERN="$OURCYGPATTERN|($GRADLE_CYGPATTERN)"
    fi
    # Now convert the arguments - kludge to limit ourselves to /bin/sh
    i=0
    for arg in "$@" ; do
        CHECK=`echo "$arg"|egrep -c "$OURCYGPATTERN" -`
        CHECK2=`echo "$arg"|egrep -c "^-"`                                 ### Determine if an option

        if [ $CHECK -ne 0 ] && [ $CHECK2 -eq 0 ] ; then                    ### Added a condition
            eval `echo args$i`=`cygpath --path --ignore --mixed "$arg"`
        else
            eval `echo args$i`="\"$arg\""
        fi
        i=$((i+1))
    done
    case $i in
        (0) set -- ;;
        (1) set -- "$args0" ;;
        (2) set -- "$args0" "$args1" ;;
        (3) set -- "$args0" "$args1" "$args2" ;;
        (4) set -- "$args0" "$args1" "$args2" "$args3" ;;
        (5) set -- "$args0" "$args1" "$args2" "$args3" "$args4" ;;
        (6) set -- "$args0" "$args1" "$args2" "$args3" "$args4" "$args5" ;;
        (7) set -- "$args0" "$args1" "$args2" "$args3" "$args4" "$args5" "$args6" ;;
        (8) set -- "$args0" "$args1" "$args2" "$args3" "$args4" "$args5" "$args6" "$args7" ;;
        (9) set -- "$args0" "$args1" "$args2" "$args3" "$args4" "$args5" "$args6" "$args7" "$args8" ;;
    esac
fi

# Split up the JVM_OPTS And GRADLE_OPTS values into an array, following the shell quoting and substitution rules
function splitJvmOpts() {
    JVM_OPTS=("$@")
}
eval splitJvmOpts $DEFAULT_JVM_OPTS $JAVA_OPTS $GRADLE_OPTS
JVM_OPTS[${#JVM_OPTS[*]}]="-Dorg.gradle.appname=$APP_BASE_NAME"

exec "$JAVACMD" "${JVM_OPTS[@]}" -classpath "$CLASSPATH" org.gradle.wrapper.GradleWrapperMain "$@"

